Do Differentiable Simulators Give Better Policy Gradients?

Differentiable simulators promise faster computation time for reinforcement learning by replacing zeroth-order gradient estimates of a stochastic objective with an estimate based on first-order gradients. However, it is yet unclear what factors decide the performance of the two estimators on complex landscapes that involve long-horizon planning and control on physical systems, despite the crucial relevance of this question for the utility of differentiable simulators. We show that characteristics of certain physical systems, such as stiffness or discontinuities, may compromise the efficacy of the first-order estimator, and analyze this phenomenon through the lens of bias and variance. We additionally propose an $\alpha$-order gradient estimator, with $\alpha \in [0,1]$, which correctly utilizes exact gradients to combine the efficiency of first-order estimates with the robustness of zero-order methods. We demonstrate the pitfalls of traditional estimators and the advantages of the $\alpha$-order estimator on some numerical examples.

==> body/benefits_of_stoch.tex <==
%!TEX root = ../icml_main.tex

\kzcomment{we might need some transition to this subsection.}

\subsection{Benefits of Stochasticity}

\kzcomment{KZ to edit}

\kzcomment{shall we incorporate this in intro? maybe titled ``Fallacies of Differentiable RL for Physical Systems''?}

Problems in RL are often stochastic by nature; for instance, the policy optimization objective involves a distribution over initial states \kzcomment{but also system transition dynamics, right?}. However, even if we want to solve a deterministic optimization problem through differentiable simulation (e.g. trajectory optimization from fixed initial state), we argue that it is better to regularize the problem through considering a stochastic objective. This argument better grounds the utility of our work for differentiable simulation, which has mainly focused on performing deterministic gradient descent.

We base this argument on randomized smoothing \cite{duchi2,suh2021bundled}. The stochastic objective can be interpreted as a smoothed version of the original objective, as the expectation can be interpreted as convolution between the original function and the probability density  (e.g. a Gaussian density results in Gaussian smoothing) Such smoothing schemes have been popular for improving convergence rates in non-smooth optimization \cite{nesterov1}, but the change in landscape can fundamentally change where gradient descent converges to.
\kzcomment{still, until this point, it seems that we have not introduced the examples in detail enough, so that readers can understand (but we use them directly in the following bullets). shall we find a way to introduce them, or at least one of them, when introducing our ``Fallacies'' in Intro?}

\begin{itemize}
\item \textbf{Smoothing Local Minima}. As noted in \cite{duchi1,suh2021bundled,metz2021gradients}, smoothing can alleviate some of the high-frequenecy local minima present in the optimization landscape. For instance, the small discontinuity in the right side of Fig.\ref{fig:systems}.B is filtered by Gaussian smoothing.
\item \textbf{Escaping Flat Regions}. In systems of Fig.\ref{fig:systems}, the gradients in some of the regions can be completely flat. This stalls progress of gradient descent. The stochastic objective, however, still has non-zero gradient as some samples escape the flat regions and provide an informative direction of improvement.
\item \textbf{Encoding Robustness.}
In addition, stochasticity can encode robustness. In Fig.\ref{fig:systems}.C, following the gradient to increase the transferred momentum causes the ball to miss the pivot completely and land in a region with high cost. On the other hand, the stochastic objective has a local minima within the safe region, as the samples provide information about missing the pivot.
\end{itemize}
 

==> body/discontinuities.tex <==
%!TEX root = ../icml_main.tex

\subsection{Physical Systems with Discontinuities}

While discontinuities may seem uncommon, the simplest physical systems can display discontinuous behavior due to presence of constraints. Examples of such systems are given in Fig.\ref{fig:systems}. We note that these systems are not merely pathologies, but abstractions of more complicated examples that are common in RL involving physical systems. In particular, contact-rich problems in intuitive physics, or robotic manipulation (e.g. dexterous in-hand manipulation) may have discontinuities due to the aforementioned reasons.

==> body/interpolation_old.tex <==
%!TEX root = ../icml_main.tex

\section{}

Previous examples give us insight on which landscapes are better fit for first-order, and which are better fit for zero-order. However, the choice of which to use can depend on the local characteristics of the landscape, such as distance to the nearest discontinuous manifold, and the strength of that discontinuity. In this section, we show that we can interpolate between the two gradients based on a probabilistic bound on the bias of the first-order estimator. We consider linear interpolation, 
\begin{definition}
    We define the Alpha-Order Batched Gradient (AoBG) and Alpha-Order Expected Gradient (AoEG) and the  as follows:
    \begin{align*}
        \nabbaralpha F(\btheta) & = \alpha \nabbarone F(\btheta) + (1-\alpha) \nabbarzero F(\btheta) \\
        \nabalpha F(\btheta) & = \alpha\nabone F(\btheta) + (1-\alpha) \nabzero F(\btheta).    
    \end{align*}
\end{definition}
Given $n$ sampled trajectories, we propose an algorithm for selecting $\alpha$. Ideally, one would choose $\alpha$ to minimize the analysis

\subsection{Gradient Interpolation}


We can easily confirm the following lemma that when the two estimators are interpolated, the bias and variance can be computed as follows.\mscomment{this lemma feels too obvious to waste space on}
\begin{lemma}
    If the two estimators are uncorrelated, the bias and variance of the two estimators are as follows:
    \begin{align*}
        \Bias(\nabbaralpha F(\btheta)) & = \alpha \Bias(\nabbarone F(\btheta)) + (1-\alpha) \Bias(\nabbarzero F(\btheta)) \\
        \Variance(\nabbaralpha F(\btheta)) & = \alpha^2 \Variance(\nabbarone F(\btheta)) + (1-\alpha)^2 \Variance(\nabbarzero F(\btheta))         
    \end{align*}
\end{lemma}
\mscomment{second inequality seems false because the two quantitiies are dependend}\tscomment{important that the samples used to compute both are independent of each other. Then it should be true?}
\subsection{Bias-Variance Tradeoff}
How do we choose $\alpha$ to tradeoff bias and variance in a sensible way, and according to which criteria? The answer is not so straightforward because there are two competing objectives of minimizing both. Although schemes such as weighting (scalarization) is possible, the weight of scalarization is often difficult to choose. 
We instead choose to frame our selection problem with that of constrained minimization, and allow minor violations of unbiasedness up to a certain threshold, while minimizing the variance as the cost.
\begin{equation}
\begin{aligned}
    \min_\alpha & \quad \Variance(\nabbaralpha F) 
  \quad  \text{s.t.}  \quad \Bias(\nabbaralpha F) \leq \gamma
    \label{eq:constraint}
\end{aligned}
\end{equation}

\subsection{Bernstein Bounds for Confidence Interval}
The constraint-based formulation gives us insights of how to choose $\alpha$; but in order to implement it, we would require the bias and variance of both FoBG and ZoBG. While the empirical variance can be used for variance, the bias is difficult to compute.

To characterize the bias term, we use the result of ZoBG $\hat{\nabla}^0_{\btheta} F(\btheta)$, an unbiased yet high-variance estimator, as a probabilistic proxy to $\nabla_{\btheta} F(\btheta)$. Then, the difference between the FoBG and the ZoBG can serve a probabilistic estimate of the bias of the FoBG $\hat{\nabla}^1_{\btheta} F(\btheta)$. For this purpose, we first construct confidence bounds using Bernstein's inequality \cite{matrixconcentration}, a finite-sample concentration result.

\iffalse
In other words,
\begin{equation}\small
    \begin{aligned}
        \|\hat{\nabla}^1_{\btheta} F(\btheta) - \hat{\nabla}^0_{\btheta} F(\btheta)\|_2 \xrightarrow[]{a.s.} &
        \;\textbf{Bias}(\hat{\nabla}^1_{\btheta} F(\btheta))\\
        =& \;\|\hat{\nabla}^1_{\btheta} F(\btheta) - \nabla_{\btheta} F(\btheta)\|_2
    \end{aligned}
\end{equation}
\fi 


% Put this here because double-column figures behave super weirdly.
\begin{figure*}[thpb]
\centering\includegraphics[width = 1.0\textwidth]{Figures/pagewide_front.png}
\vskip -0.1 true in
\caption{Left Column: Ball with Wall example. Leftmost figure indicates the variance, bias, landscape, and $\alpha$ value of our algorithm. In the third row, the triangle is the initial point, and red/blue/green stars are the optimum achieved by FoBG, ZoBG, and AoBG respectively. Right: Iteration vs. Cost plot of different gradients. Right column: Same plot is repeated for the momentum transfer example. Standard deviation is plotted 10 fold for visualization.}
\label{fig:simplesystems}
\vskip -0.1 true in
\end{figure*}


\mscomment{Bernstein uses the true variance, not the empirical. You need to make this an empirical bernstein}
\begin{lemma}[Bernstein] Given the empirical variance $\hat{\sigma}_n^2$ and an upper bound on the per-sample \mscomment{deviation} $L$:
    \begin{align*}
        &\hat{\sigma}^2_N := \textstyle\frac{1}{N} \sum_{i=1}^N \| \nabhatzero F_i - \nabbarzero F\|^2_2\\ 
        &\|\nabhatzero F_i - \nabzero  F\|_2\leq L,
    \end{align*}
    the finite-sample deviation satisfies the following concentration inequality:
    \begin{align*}\small
        \mathbb{P}\bigg(\|\nabla_{\btheta} F - \hat{\nabla}^0_{\btheta} F \|_2 \geq \varepsilon\bigg) \leq (n + 1) \cdot \exp
        \bigg(\frac{-\varepsilon^2 N / 2}{\hat{\sigma}^2_N + L\varepsilon/(3\varepsilon)}\bigg)
    \end{align*}
    \begin{proof}
        Matrix Bernstein's Inequality for sums  \cite{matrixconcentration} can be easily modified for means. We substitute the expected variance with the empirical variance.
    \end{proof}
\end{lemma}

\subsection{Chance-Constrained Formulation}
The confidence interval allows us to compute a probabilsitic bound on the bias of AoBG, given the observed difference between the FoBG and ZoBG.

\begin{theorem}
    With probability $\delta$, the bias of AoBG is bounded by
    \begin{align*}
        \normalfont{\textbf{Bias}}(\hat{\nabla}^\alpha_{\btheta} F) \leq \varepsilon + \alpha \|\hat{\nabla}^1_{\btheta} F - \hat{\nabla}^0_{\btheta} F\|
    \end{align*}
    where $(\varepsilon,\delta)$ are the confidence interval and the probability that satisfy Bernstein's inequality.
\end{theorem}
\begin{proof}
    Appendix.
\end{proof}
 
As we can now only guarantee this with probability, one interpretation is that the problem now becomes a chance-constrained modification of Eq.\ref{eq:constraint}.

\begin{align*}
        \min_\alpha & \quad \textbf{Var}(\nabla^\alpha_{\btheta} F ) \\
        \text{s.t.} & \quad \mathbb{P}(\textbf{Bias}(\nabla^\alpha_{\btheta} F) \leq \gamma) \geq \delta     
        \label{eq:chanceconstraint}
\end{align*}

\subsection{The Interpolation Algorithm}

Now we have all the pieces to formulate a tractable formulation for the constrained optimization problem of Eq.\ref{eq:constraint}:
\begin{align}
        \min_\alpha & \quad \alpha^2 \sigma_1^2 + (1-\alpha)^2 \sigma_0^2 \\
        \text{s.t.} & \quad \varepsilon + \alpha \underbrace{\|\hat{\nabla}^1_{\btheta} F - \hat{\nabla}^0_{\btheta} F\|}_B \leq \gamma 
    \label{eq:tractableform}
\end{align}

where $\sigma^2$ are the empirical variances, and $B$ is the difference between the FoBG and the ZoBG. Eq.\ref{eq:tractableform} is a trivial QP with an analytical solution: complementary slackness would indicate that the optimum is achieved at the optimum of the unconstrained problem if that optimum is feasible, and at the boundary of the feasible set if not. 

\begin{lemma}\normalfont 
    The optimum of the unconstrained problem of Eq.\ref{eq:tractableform} is
    \begin{equation}\small
        \bar{\alpha} = \frac{\sigma_0^2}{\sigma_1^2 + \sigma_0^2},
        \label{eq:unconstrained}
    \end{equation}
    and the solution to Eq.\ref{eq:tractableform} is given by 
    \begin{equation}\small
        \alpha^* = \begin{cases}
            \bar{\alpha} & \text{ if } \quad \bar{\alpha} B \leq \gamma - \varepsilon \\ 
            \frac{\gamma-\varepsilon}{B} & \text{ else } 
        \end{cases}
    \end{equation}
    \begin{proof}
        Appendix A.6.
    \end{proof}
\end{lemma}

The unconstrained formulation is equivalent to the inverse variance weighting formulation and equivalent to the formulas presented in \cite{parmas,pathologies}.

Finally, note that Eq.\ref{eq:tractableform} is infeasible if $\varepsilon > \gamma$, which suggests that there are simply not enough confidence to meet the bounds $\gamma$ with the given probability $\delta$. In this case, as no certification of the bias of FoBG can be made, we resort to fully trusting ZoBG (i.e. $\alpha=0$). Asymptotically as sample size $N\rightarrow 0$, the confidence interval $\varepsilon\rightarrow 0$, which would indicate that the problem becomes feasible.

\begin{algorithm}[thpb]
   \caption{ComputeAoBG}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} FoBG $\hat{\nabla}^1_x F$, ZoBG $\hat{\nabla}^0_x F$
   \STATE {\bfseries Input:} Empirical variances $\sigma_1^2, \sigma_0^2$
   \STATE {\bfseries Input:} Bias threshold $\gamma$, probability $\delta$

   \STATE Compute Confidence Interval $\varepsilon$.
   \IF{$\varepsilon > \gamma$}
        \STATE $\alpha = 0$ 
   \ELSE
        \STATE Compute $\bar{\alpha}$ (Eq.\ref{eq:unconstrained})
        \STATE Compute $B=\|\hat{\nabla}^1_x F - \hat{\nabla}^0_x F\|$
        \IF{$\bar{\alpha} B \leq \gamma - \varepsilon$}
            \STATE $\alpha = \bar{\alpha}$
        \ELSE
            \STATE $\alpha = (\gamma - \varepsilon) / B$
        \ENDIF
   \ENDIF
   \STATE {\bfseries Return:} $\alpha \hat{\nabla}^1_x F + (1-\alpha)\hat{\nabla}^0_x F$ 
\end{algorithmic}
\end{algorithm}

==> body/policy_opt.tex <==

\subsection{Motivating Example: Policy Optimization}
\tscomment{How should we best present this? Full proof seems unnecessary. One simple way is just to show that the ZoBG equivalent to the usual log expression, and also show say this encompasses trajectory optimization.}
\begin{example}
    \normalfont \textbf{Policy Gradient Theorem} 
    Consider the policy optimization problem where the policy is parametrized by decision variables $\theta$. Let $g=\pi(x,\theta)$ be the output of the policy given state $x$. The objective is to minimize the outer value function of the parametrized policy, $V$:
    \begin{equation}\small
        \begin{aligned}
            \min_\theta & \; \mathbb{E}_{x\sim\rho,\bar{w}_t\sim p}\bigg[V(x,\theta,\bar{w}_t) = c_T(x_T) + \sum^{T-1}_{t=0} \gamma^t c(x_t, u_t)\bigg] \\
            \text{s.t.} & \; x_0 = x \\
                        & \; x_{t+1} = f(x_t, u_t) \\
                        & \; u_t = \pi(x_t,\theta) + w_t \quad w_t\sim \mathcal{N}(0,\sigma^2\mathbf{I})
        \end{aligned}        
    \end{equation}
    The ZoBG for this problem can be written as 
    \begin{equation}\small
        \hat{\nabla}^0_\theta F(\theta) = \frac{1}{NM}\sum^M_{i=1}\sum^N_{j=1}\frac{\nabla_\theta \pi(x_i,\theta)^\intercal}{N \sigma} \big[V(x_i,\theta,w_j)w_j\big]
        \label{eq:pozobg}
    \end{equation}
    where $i$ is index for sampling through initial states, and $j$ is the index for sampling through the noise. Note that $V(x_i,\theta,w_j)$ can be obtained from rolling out the simulation, and $\nabla_\theta \pi(x_i,\theta)$ only requires gradient of the policy, and thus no ability to differentiate through the simulation is necessary. The estimator obtained using the ZoBG is equal to that obtained by the popular policy gradient theorem \cite{reinforce}:
    \begin{equation}\small
        \nabla_\theta \mathbb{E}_{x,\bar{w}}\big[V(x,\theta,\bar{w})\big] = \mathbb{E}_{x,\bar{w}}[V(x,\theta,\bar{w}) \nabla_\theta \log p_\pi(x,\theta)]
        \label{eq:pg}
    \end{equation}
    where $p_\pi$ is the distribution induced by the policy (i.e. $p_\pi=\mathcal{N}(\pi(x,\theta),\sigma^2\mathbf{I})$. We refer to Appendix \ref{sec:a4} for proof. The FoBG for this problem utilizes derivatives of the dynamics, policy, and the cost, and is referred to as the \textit{analytical policy gradient} in \cite{brax}. 
\end{example}



==> body/preliminaries.tex <==
%!TEX root = ../icml_main.tex


\section{Preliminaries} 
\textbf{Technicalities.} Throughout, all functions are assumed to be Borel-measurable so that expectations are defined \mscomment{cite}. In many cases, we will consider expectations of functions defined almost-every where, e.g. expectations of derivatives of Lipschitz functions. We define these expectations so that the weak law of large numbers hold (see appendix. ) 

\textbf{Stochastic Optimization.}
In stochastic optimization, the goal is to minimize a stochastic objective $F(\theta)=\Exp_{x\sim \rho}\mathbb{E}_{w\sim p}[f(\theta,w,x)]$,
\begin{equation}
    \min_{\theta} F(\theta) = \min_{\theta} \mathbb{E}_{w\sim p} \big[f(\theta,w)\big],
\end{equation}
where $\theta\in\mathbb{R}^n$ is the decision variable, $w\in\mathbb{R}^m$ are random variables with density $p$, ad $f:\R^{n} \times \R^m \to \R$. We assume that $f(\theta,w)$ is \textit{linearly separable} in $\theta$ and $w$.
\begin{assumption}\label{assumption:separable}
For functions $\gin:\mathbb{R}^n\rightarrow\mathbb{R}^m$ and $\gout: \R^n \to \R$ and smoothing parameter $\sigma > 0$, 
    \begin{align}
    f(\theta,w) = \gout(\gin(\theta) + \sigma w).
    \end{align}
\end{assumption}
Separability is quite a mild condition \mscomment{explain}. 
For simplicity, we further assume $w$ is Gaussian; in principle, our results extend to other light-tailed distributions with Lebesgue density. 
\begin{assumption} We assume that $w$ is drawn from the Gaussian distribution $p = \calN(0,I_n)$. 
\end{assumption}
In order to perform such a minimization, a central quantity of our interest is the gradient of the stochastic objective:
\begin{equation}
    \nabla_x F(x) = \nabla_x \mathbb{E}_{w\sim p}[f(x,w)] \label{eq:nabla_F}
\end{equation}
 We say a function $g:\R^d \to R$ has \emph{subexponential growth} if there exists constants $c_1,c_2 > 0$ such that $|g(x)| \le c_1(1+ e^{c_2\|x\|})$. To ensure $F(x)$ and $\nabla_x F(x)$ are well-defined, we assume the following:
 \begin{assumption} For all $x \in \R^d$, $\gin(x)$ is differentiable, and $\gout(\cdot)$ has subexponential growth. 
 \end{assumption}
 Importantly, $\gout(\cdot)$ \emph{need not be continuous.}

 \begin{example}[toy]\msedit{toy example here}
 \end{example}


\subsection{Gradient Estimators. } If the first-order gradient $\nabla_x f(x,w)$ is available, one may directly sample and average them to estimate the gradient of the stochastic objective.
\begin{definition} Given a single first-order stochastic gradient    \begin{equation}\small
        \nabla^1_x F_i(x) = \nabla_x f(g(x) + w_i),
    \end{equation}
    we define  first-order batched gradient $\hat{\nabla}^1_x F(x)$ (\fobg) and first-order expected gradient $\nabla^1_x F(x)$ (\foeg) as follows:
    \begin{equation}\nonumber
        \begin{aligned}
        \hat{\nabla}_x^1 F(x) & \coloneqq \textstyle \frac{1}{N} \sum^N_{i=1} \nabla^1_x F_i(x)\\
        \nabla_x^1 F(x) & \coloneqq \mathbb{E}_{w_i\sim p} \nabla^1_x F_i(x) = \Exp_{w_1,\dots,w_N \sim p}[\hat{\nabla}_x^1 F(x) ]
        \end{aligned}
    \end{equation}
\end{definition}

Note the hat notation on the gradient to denote that \fobg{} is a Monte-Carlo estimate of \foeg{}. The \fobg{} is also referred to as the reparametrization gradient \cite{kingma}. Again, care must be taken to define the \foeg{} since $\nabla f(x,w)$ need not be defined everywhere. As noted above, we choose our definition so that the law of large numbers holds (see \msedit{appendix}). 



Unlike the first-order estimator, the zeroth-order estimator \cite{reinforce, nesterov2, ghadimilan} does not rely on any analytical gradients, but rather, requires only samples of the function itself to estimate the gradient.
\begin{definition} \normalfont 
    Given a zeroth-order stochastic gradient
    \begin{equation}\small
        \nabla^0_x F_i(x) = \textstyle \frac{\nabla_x g(x)^\intercal}{\sigma} f(g(x) + \sigma w_i)w_i,
    \end{equation}
    we define the zeroth-order batched gradient $\hat{\nabla}^0_x $ (ZoBG) and zeroth-order expected gradient $\nabla^0_x$ (ZoEG) as
    \begin{equation}\small\nonumber
        \begin{aligned}
        \hat{\nabla}^0_x F(x) & \coloneqq \textstyle \frac{1}{N}\sum^N_{i=1} \nabla^0_x F_i(x) \\   
            \nabla^0_x F(x) & \coloneqq \mathbb{E}_{w_i\sim p} \nabla^0_x F_i(x) = \Exp_{w_1,\dots,w_N \sim p}[\hat{\nabla}^0_x F(x) ].
        \end{aligned}
    \end{equation}
\end{definition}
    The ZoBG is also referred to as the REINFORCE \cite{reinforce}, or the likelihood gradient. 

\subsection{Motivating Example: Policy Optimization}

\begin{example}
    \normalfont \textbf{Policy Gradient Theorem} 
    Consider the policy optimization problem where the policy is parametrized by decision variables $\theta$. Let $g=\pi(x,\theta)$ be the output of the policy given state $x$. The objective is to minimize the outer value function of the parametrized policy, $V$:
    \begin{equation}\small
        \begin{aligned}
            \min_\theta & \; \mathbb{E}_{x\sim\rho,\bar{w}_t\sim p}\bigg[V(x,\theta,\bar{w}_t) = c_T(x_T) + \sum^{T-1}_{t=0} \gamma^t c(x_t, u_t)\bigg] \\
            \text{s.t.} & \; x_0 = x \\
                        & \; x_{t+1} = f(x_t, u_t) \\
                        & \; u_t = \pi(x_t,\theta) + w_t \quad w_t\sim \mathcal{N}(0,\sigma^2\mathbf{I})
        \end{aligned}        
    \end{equation}
    The ZoBG for this problem can be written as 
    \begin{equation}\small
        \frac{1}{NM}\sum^N_{i=1} \sum^M_{j=1} V(x^i_1, \theta, w^j) \sum^H_{k=1} \frac{1}{\sigma} \nabla_\theta \pi(x^i_k,\theta)^\intercal w_k^j
        \label{eq:pozobg}
    \end{equation}
    where $i$ is sample index for initial states, $j$ for noise trajectory, and $k$ for time. Note that $V(x^i_1, \theta, w^j)$ can be obtained from rolling out the simulation, and $\nabla_\theta \pi(x^i_k,\theta)$ only requires gradient of the policy, and thus no ability to differentiate through the simulation is necessary. The estimator obtained using the ZoBG is equal to that obtained by the popular policy gradient theorem \cite{reinforce}:
    \begin{equation}\small
        \nabla_\theta \mathbb{E}_{x,\bar{w}}\big[V(x,\theta,\bar{w})\big] = \mathbb{E}_{x,\bar{w}}[V(x,\theta,\bar{w}) \nabla_\theta \log p_\pi(x,\theta)]
        \label{eq:pg}
    \end{equation}
    where $p_\pi$ is the distribution induced by the policy (i.e. $p_\pi=\mathcal{N}(\pi(x,\theta),\sigma^2\mathbf{I})$. We refer to Appendix \ref{sec:a4} for proof. The FoBG for this problem utilizes derivatives of the dynamics, policy, and the cost, and is referred to as the \textit{analytical policy gradient} in \cite{brax}. 
\end{example}



==> body/related_work.tex <==
%!TEX root = ../icml_main.tex

\subsection{Related Work}
\tscomment{Kaiqing and I will dump related work here, will organize later.}
\kzcomment{as per terry's suggestion in the morning, let's shove them into intro?}

\paragraph{Stochastic Optimization in Discontinuities}
\paragraph{Differentiable Simulation}
many efforts are underway to replace existing zero-order RL algorithms with first-order gradients (termed ``differentiable RL''), which has shown convincing results in terms of decrease in computation time \cite{plasticinelab,brax,deluca}.
\paragraph{Interpolating Gradients} Combining first-order gradients and zero-order gradients have been attempted in previous works \cite{stochasticcompuationgraph,parmas,pathologies,montecarlo}, but most works only consider the setting where both estimators are unbiased. Thus, only the variance is used as a weighting criteria. As our work studies the case where the first-order estimator is biased, we extend the minimum-variance interpolation problem by adding a chance constraint on the bias of the interpolated gradient. 

